The Pointillist Family of Multitarget Tracking Filters

The family of pointillist multitarget tracking filters is defined to be the class of filters that is characterized by a joint target-measurement finite point process. The probability generating functional (PGFL) of the joint process is derived directly from the probabilistic structure of the tracking problem. PGFLs exemplify the analytic combinatoric method applied to the measurement to target assignment problems that are fundamental to the tracking problem. It is shown that multi-hypothesis tracking (MHT), joint probabilistic data association (JPDA), and many other now-classic tracking filters can be derived via PGFLs, and thus are members of the family of pointillist filters. When one or more of the target processes are dimensionally compatible, targets can be superposed. It is shown that the classic MHT filter for superposed targets is closely related to the multi-Bernoulli filter. A technique is presented for deriving the functional derivatives by ordinary differentiation, and both exact and approximate methods for evaluating the ordinary derivatives are discussed.

==> tablesForFigures.tex <==
\begin{table*} 
	\centering
	\tiny	
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}	
		\hline
		\label{tableOfPointillistFilters}
		\bf{Filter Name} & \bf{PGFL Notation} & \bf{Joint Target-Measurement PGFL} & \bf{Ref.} & \bf{Target} \bf{Model} & \bf{Clutter} & \bf{Missed} &  \bf{Super-} \Tstrut\\ 
		\ &  \ & \ & \bf{Eqn.} & \ & \  & \bf{Detection} &  \bf{position} \Bstrut  \\  \hline		
		\bf{Bayes-Markov} & $\Psi_{\text{BM}}(h,g)$ & $\int_S \int_Y h(x) g(y) \mu(x) p(y|x) \,dy\,dx$ &(\ref{BayesMarkov})  & $ =1$ point target & No & No & No \Tstrut \Bstrut \\
		\,\,\,\textit{Missed Detections} & $\Psi_{\text{BMD}}(h,g)$ & $\int_S h(x) \mu(x)\, G_{M|x}^{\text{BMD}}\big( \int_Y  g(y) p(y|x) \,dy\big) \, dx$ &(\ref{BayesMarkovMissedDet}) & $=1$ point target & No & Standard  & No   \Bstrut\\	
		\,\,\,\textit{Missed Detections} & $\Psi_{\text{BME}}(h,g)$ & $\int_S h(x) \mu(x)\, G_{M|x}\big( \int_Y  g(y) p(y|x) \,dy\big) \, dx$ & (\ref{extendedBayesianTarget}) & $=1$ ext. target & No & General$^5$ & No  \Bstrut \\ 
		\,\,\,\,\,\,\textit{and Extended Target} &  \ & \ & \ & \ & \  & \ & \   \Bstrut \\ \hline
		\bf{PMHT} &  \ & \ & \ & \ & \ & \  & \  \Tstrut \Bstrut \\
		\,\,\,\textit{Without Superposition} & $\Psi_{\text{PMHT}}(h_1,\dots,h_n,g)$ & $\prod_{i=1}^{n}\Psi_{\text{BMD}(i)}^{\text{PPP}}(h_i,g)$  & (\ref{PGFLforPMHT}) & $=n$ ext. targets & No$^1$  & No$^8$  & No \Bstrut \\
		\,\,\,\textit{With Superposition} & $\Psi_{\text{PMHTS}}(h,g)$ & $\prod_{i=1}^{n}\Psi_{\text{BMD}(i)}^{\text{PPP}}(h,g)$  & (\ref{SuperposedPMHT}) & $=n$ ext. targets & No$^1$  & No$^8$ & Yes \Bstrut \\ \hline
		\bf{PDA} &  \ & \ & \ & \ & \ &\  & \ \Tstrut \Bstrut \\
		\,\,\,\textit{Without Gating} &  $\Psi_{\text{PDA}}^{\text{noGate}}(h,g)$ & $\Psi_{\text{BMD}}(h,g)\,\Psi_{C}^{\text{PPP}}(g)$&  (\ref{PDAnoGating}) & $=1$  point target & Poisson  & Standard  & No  \Bstrut \\
		\,\,\,\textit{With Gating} & $\Psi_{\text{PDA}}(h,g)$ & $\Psi_{\text{BMD}}^{\text{gated}}(h,g)\,\Psi_{C}^{\text{PPPgated}}(g)$ &  (\ref{PDAwithGating}) & $=1$  point target & Poisson  & Standard & No  \Bstrut	\\
		\,\,\,\textit{Extended Target} & $\Psi_{\text{PDAE}}(h,g)$ & $\Psi_{\text{BME}}(h,g)\,\Psi_{C}^{\text{PPP}}(g)$ & (\ref{PDAwithExtendedTarget}) &	$=1$  ext. target & Poisson & General$^5$  & No \Bstrut \\\hline
		\bf{JPDA} &  \ & \ & \ & \ & \  & \ & \ \Tstrut \Bstrut \\
		\,\,\,\textit{Without Superposition} & $\Psi_{\text{JPDA}}(h_1,\dots,h_n,g)$ & $\prod_{i=1}^n\Psi_{\text{BMD}(i)}(h_i,g)\,\Psi_{C}^{\text{PPP}}(g)$  & (\ref{PGFLforJPDA}) & $=n$ point targets & Poisson & Standard  & No \Bstrut \\ 
		\,\,\,\textit{With Superposition} & $\Psi_{\text{JPDAS}}(h,g)$ & $\Psi_{\text{JPDA}}(h,\dots,h,g)$  &  (\ref{PGFLforJPDAS}) & $=n$ point targets & Poisson & Standard  & Yes  \Bstrut \\ \hline		
		\bf{IPDA} & $\Psi_{\text{IPDA}(h,g)}$ & $\Big( 1-\chi+\chi\,\Psi_{\text{BMD}}(h,g) \Big)\,\Psi_{C}^{\text{PPP}}(g)$  & (\ref{IPDA}) & $\le 1$ point target & Poisson & Standard & No \Tstrut \Bstrut \\ \hline
		\bf{JIPDA} &  \ & \ & \ &  \ & \ & \  & \  \Tstrut \Bstrut \\
		\,\,\,\textit{Without Gating} & $\Psi_{\text{JIPDA}}(h_1,\dots,h_n,g)$ & $\prod_{i=1}^n\Big  (1-\chi_i+\chi_i\,\Psi_{\text{BMD}(i)}(h_i,g)\Big)\,\Psi_{C}^{\text{PPP}}(g)$ & (\ref{pgflForJIPDAprocess}) & $\le n$ point targets & Poisson & Standard & No \Bstrut \\
		\,\,\,\textit{With Gating} & $\Psi_{\text{JIPDA}}^{\text{gated}}(h_1,\dots,h_n,g)$ & $\prod_{i=1}^n\Big  (1-\chi_i+\chi_i\,\Psi_{\text{BMD}(i)}^{\text{gated}}(h_i,g)\Big)\,\Psi_{C}^{\text{PPPgated}}(g)$ &  (\ref{pgflForJIPDAprocessGated}) & $\le n$ point targets & Poisson & Standard  & No \Bstrut \\		
		\,\,\,\textit{With Superposition} & $\Psi_{\text{JIPDAS}}(h,g)$ & $\Psi_{\text{JIPDA}}(h,\dots,h,g)$ &  (\ref{SuperposedJIPDAS}) & $\le n$ point targets & Poisson & Standard & Yes \Bstrut \\ \hline
		\bf{MHT}$^{2}$ & $\Psi_{\text{MHT}}(h_1,\dots,h_{n+m},g)$ & $\prod_{i=1}^n\Big(1-\chi_i+\chi_i\,\Psi_{\text{BMD}(i)}(h_i,g)\Big)$ &  (\ref{pgflForJIPDADataDriven}) & $\le n+m$  & Poisson & Standard & No \Tstrut \Bstrut \\
		\ & \ & $\times \prod_{j=1}^m \Big(1-\gamma_j+\gamma_j\,\Psi_{\text{BMD}(j)}^{\text{Data}}(h_{n+j},g)\Big)$ &  \ & point targets & \  & \ & \ \Bstrut \\	
		\ & \ & $\times \, \Psi_{C}^{\text{PPP}}(g)$  &   \ & \ & \  &  \ & \ \Bstrut \\	\hline
		\bf{Multi-Bernoulli} & $\Psi_{\text{MB}}(h,g)$ & $\prod_{i=1}^n\Big(1-\chi_i+\chi_i\,\Psi_{\text{BMD}(i)}(h,g)\Big)$	& (\ref{pgflMultiBernoulli}) & $\le n+m$  & Poisson & Standard  & Yes\Tstrut \Bstrut \\
		\ & \ & $\times \prod_{j=1}^m \Big(1-\gamma_j+\gamma_j\,\Psi_{\text{BMD}(j)}^{\text{Data}}(h,g)\Big)$  &  \ &  point targets  & \ & \ & \  \Bstrut \\
		\ & \ & $\times \, \Psi_{C}^{\text{PPP}}(g)$  &  \ & \  & \ & \ & \  \Bstrut \\ \hline
		\bf{PHD} & $\Psi_{\text{PHD}}(h,g)$ & $G_N^{\text{PPP}}\big(\Psi_{\text{BMD}}(h,g)\big)\,\Psi_{C}^{\text{PPP}}(g)$	 & (\ref{pgflPHD}) & Poisson & Poisson & Standard & Yes\Tstrut \Bstrut \\\hline
		\bf{CPHD} & $\Psi_{\text{CPHD}}(h,g)$ & $G_{N}^{\text{Cluster}}\big(\Psi_{\text{BMD}}(h,g)\big)\,\Psi_{C}^{\text{PPP}}(g)$	& (\ref{PGFLCPHD}) & Cluster & Cluster & Standard & Yes\Tstrut \Bstrut \\\hline
		\bf{Generalized PHD} & $\Psi_{\text{GenPHD}}(h,g)$ & $G_N\big(\Psi_{\text{BMD}}^{\text{gen}}(h,g)\big)\,\Psi_{C}^{\text{gen}}(g)$	 & (\ref{pgflGeneralizedPHD}) & General$^7$ & General$^6$ & General$^4$ & Yes\Tstrut \Bstrut \\ \hline	
		\bf{Joint PHD} & $\Psi_{\text{JointPHD}}(h_1,\dots,h_n,g)$ &  $\prod_{i=1}^n G_{N_i}^{\text{PPP}}\big (\Psi_{\text{BMD}}(h_i,g)\big)\,\Psi_{C}^{\text{PPP}}(g)$ & (\ref{jointPHDPGFL}) & $= n$ target groups  & Poisson & Standard$^3$  & Yes$^3$ \Tstrut \Bstrut \\ \hline 
		\bf{Joint Generalized PHD} & $\Psi_{\text{JointGenPHD}}(h_1,\dots,h_n,g)$ &  $\prod_{i=1}^n G_{N_i}^{\text{PPP}}\big (\Psi_{\text{BMD}}^{\text{gen}}(h_i,g)\big)\,\Psi_{C}^{\text{gen}}(g)$ &  (\ref{pgflJointGeneralizedPHD}) & $= n$ target groups & General$^6$ & General$^{3,4}$  & Yes$^3$\Tstrut \Bstrut \\ \hline		
	\end{tabular}
	\begin{tabular}{llllllllll}
		\	&  \ & \ & \ &  \ & \ & \  & \ & \ & \ \\
	\end{tabular}
	\caption{Overview of the pointillist family of multitarget tracking filters} 	
	\begin{enumerate}
		\item[1] Clutter is modelled as a target with high variance in the PMHT-filter
		\item[2] MHT of un-pruned and complete set of hypothesis
		\item[3] Within target groups
		\item[4] Arbitrary target-oriented measurement process 
		\item[5] Extended target measurement model
		\item[6] General finite point process clutter model
		\item[7] General finite point process target model
		\item[8] Modeled via missing data assignment weight (Expectation Maximization algorithm)
	\end{enumerate}	
\end{table*}
